The multi-wavelength view of shocks in the fastest nova V1674 Her

Classical novae are shock-powered multi-wavelength transients triggered by a thermonuclear runaway on an accreting white dwarf. V1674 Her is the fastest nova ever recorded (time to declined by two magnitudes is t_2=1.1 d) that challenges our understanding of shock formation in novae. We investigate the physical mechanisms behind nova emission from GeV gamma-rays to cm-band radio using coordinated Fermi-LAT, NuSTAR, Swift and VLA observations supported by optical photometry. Fermi-LAT detected short-lived (18 h) 0.1-100 GeV emission from V1674 Her that appeared 6 h after the eruption began; this was at a level of (1.6 +/- 0.4)x10^-6 photons cm^-2 s^-1. Eleven days later, simultaneous NuSTAR and Swift X-ray observations revealed optically thin thermal plasma shock-heated to kT_shock = 4 keV. The lack of a detectable 6.7 keV Fe K_alpha emission suggests super-solar CNO abundances. The radio emission from V1674 Her was consistent with thermal emission at early times and synchrotron at late times. The radio spectrum steeply rising with frequency may be a result of either free-free absorption of synchrotron and thermal emission by unshocked outer regions of the nova shell or the Razin-Tsytovich effect attenuating synchrotron emission in dense plasma. The development of the shock inside the ejecta is unaffected by the extraordinarily rapid evolution and the intermediate polar host of this nova.

==> Makefile <==
#
# ---=== Ultimate LaTeX astronomy paper/proposal makefile ===---
#
# Run 'make' to compile a LaTeX source and display the reulting PDF with 'okular'
# The Makefile understands 'latex'/'pdflatex' with or without 'bibtex'.
# The Makefile will apply a set of tests aiming to catch common typos, repeated words, 
# check US/British spelling and some aspects of AAS/MNRAS journal style.
#
# The Makefile assumes it is run by GNUmake and relies on external tools including cat, cut, grep, sed, awk, and okular
# 
# The originla version of this Makefile was created by Kirill Sokolovsky <kirx@kirx.net>
#
######################################################################################################
# Manual setttings that modify the makefile behaviour

# Set to "yes" if this is an arXiv sumbission (needs .bbl file) otherwise set "no" (remove .bbl file on cleanup)
#ARXIV=no
ARXIV=yes

# Display the compiled document using okular PDF viewer? (yes/no)
LAUNCH_OKULAR_PDF_VIEWER_TO_DISPLAY_COMPILED_PAPER=yes

COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT=yes

# Disable some individual tests if needed (yes/no)
TEST_SOFTWARE_TEXTSC=yes
TEST_NONASCII_CHARS=yes

######################################################################################################
# Automated setup: try hard to find the main tex file and recognize its format: PDF figure, BibTeX...
#
# Set *main.tex as the main TeX file, otherwise assume the largest TeX file is the main TeX file
TEXFILE_BASENAME := $(shell if [ -f *main.tex ];then ls *main.tex ;else ls -S *.tex ;fi | head -n1 | sed 's:.tex::g')

PDFTEX := $(shell cat *.tex | cut -f1 -d"%" | grep 'includegr' | grep --quiet -e '.pdf' -e '.png' && echo 'yes' )
BIBTEX := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet 'bibliographystyle' && echo 'yes' )

BIBFILENAME := $(shell cat *.tex | cut -f1 -d"%" | grep 'bibliography{' | head -n1 | awk -F'bibliography{' '{print $$2}' | awk -F'}' '{print $$1".bib"}')

MODIFY_BIBFILE_ULTRACOMPACT_REF := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'bibliographystyle.mnras_shortlisthack' -e 'bibliographystyle.supershort_numbers_oneline' && echo 'yes' )

MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'mnras' && echo 'yes' )

AAS_MANUSCRIPT_REQUIRING_US_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'aastex' && echo 'yes' )

ANY_KNOWN_SOFTWARE_MENTIONED := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'IRAF' -e 'MIDAS' -e 'AIPS' -e 'CASA' -e 'DS9' -e 'ds9' -e 'VaST' -e 'HEASoft' -e 'HEASOFT' -e 'HEAsoft' -e 'Fermitools' -e 'Difmap' -e 'difmap' -e 'DiFx' -e 'SExtractor' -e 'sextractor' -e 'PSFEx' -e 'psfex' && echo 'yes' )

IS_SWIFT_UVOT_MENTIONED := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'Swift' && cat *.tex | cut -f1 -d"%" | grep --quiet -e 'UVOT' && echo 'yes' )


all: info clean check_utf8 check_spell check_no_whitespace check_coma_instead_of_period check_extra_white_space try_to_find_duplicate_words shorten_journal_names_bib check_british_spelling check_us_spelling check_gamma_ray_math_mode check_software_small_capitals check_swift_uvot_lowercase_filternames check_units check_consistent_unbreakable_space_size_UT check_phrasing check_filenames_good_for_arXiv  $(TEXFILE_BASENAME).pdf  check_for_bonus_figures display_compiled_pdf


info: $(TEXFILE_BASENAME).tex
	@echo "Starting the ultimate LaTeX Makefile"
	@echo "TEXFILE_BASENAME= "$(TEXFILE_BASENAME)
ifeq ($(BIBTEX),yes)
	@echo "BIBFILENAME= "$(BIBFILENAME)
else
	@echo "No BibTeX, fine"
endif

clean: 
ifeq ($(ARXIV),yes)
	# do not remove .bbl file for arXiv submission
	rm -f $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~
else
	# remove .bbl file and everything else
	rm -f $(TEXFILE_BASENAME).bbl  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~
endif

check_utf8: $(TEXFILE_BASENAME).tex
ifeq ($(TEST_NONASCII_CHARS),yes)
	#
	# Display any non-ASCII UTF8 characters higlighting them with color.
	# (If this check fails, but you see no color in the output -
	# the non-ASCII character is masquerading as white space and
	# you may need to select text with mouse to see the offending character.)
	#
	@echo "Searching for non-ASCII characters in TeX file"
	{ LC_ALL=C grep --color=always '[^ -~]\+' *.tex && exit 1 || true; }
	#{ LC_ALL=C grep --color=always '[^ -~]\+' $(TEXFILE_BASENAME).tex && exit 1 || true; }
	# Check that the TeX file type is not Unicode - but that may miss some stray Unicode character
	file *.tex | { grep -e 'Unicode' -e 'ISO-8859' && exit 1 || true; }
	#file $(TEXFILE_BASENAME).tex | { grep Unicode && exit 1 || true; }
ifeq ($(BIBTEX),yes)
	@echo "Searching for non-ASCII characters in BibTeX file"
	{ LC_ALL=C grep --color=always '[^ -~]\+' $(BIBFILENAME) && echo 'ERROR: Unicode character in .bib file' && exit 1 || true; }
endif
endif


check_spell: $(TEXFILE_BASENAME).tex
	# Case-insensitive search
	# sed 's/[^ ]*.eps[^ ]*//ig'   is to make sure figure filenames are ignored
	cat *.tex | sed 's:the A config::g' | sed 's:binary tree::g' | sed 's/[^ ]*.eps[^ ]*//ig' | { grep --color=always --ignore-case -e 'compliment' -e 'complimented' -e 'ile up' -e 'ile~up' -e '\bcan will\b' -e '\bmay can\b' -e '\bmay will\b' -e '\ba the\b' -e '\bthe a\b' -e '\bwhited\b' -e '\bneutrons star\b' -e '\bhotpot\b' -e '\brang\b' -e 'has be seen' -e 'synchroton' -e '\bhight\b' -e 'far from being settled' -e 'recourses' -e '\bwile\b' -e 'will allows' -e '\btree\b' -e '\ban new\b' && exit 1 || true; }
	# Case-sensitive search
	cat *.tex | sed 's:the A config::g' | { grep --color=always -e 'x-ray' -e ' tp ' && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | sed -ie 's/\\[A-Za-z0-9]* / /g' | { grep --color=always 'countrate' && echo "SHOULD BE count rate" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat *.tex | cut -f1 -d"%" | { grep --color=always '\bgenue\b' && echo "SHOULD BE genuine" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always '\bTHe\b' && echo "SHOULD BE the" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'maid' && echo "DID YOU MEAN made ?" && exit 1 || true; }
	# 'substraction' is a rare synonym for 'embezzlement' https://www.merriam-webster.com/dictionary/substraction
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'substraction' && echo "DID YOU MEAN subtraction ?" && exit 1 || true; }
	# and the all-time classic
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'redshit' && echo "DID YOU MEAN redshift ?" && exit 1 || true; }
	# 'common-envelop' is not your ordinary package for a letter
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case '\bcommon-envelop\b' && echo "DID YOU MEAN common-envelope ?" && exit 1 || true; }
	# ' on Fig'
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case '\bon Fig' && echo "DID YOU MEAN in Fig... ?" && exit 1 || true; }
	#
	# 'number if'
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case '\bnumber if\b' && echo "DID YOU MEAN number of ?" && exit 1 || true; }
	# novae instead of novas, unless it looks like software name 'NOVAS' - a popular astrometry library
	cat *.tex | cut -f1 -d"%" | sed -e 's/textsc{[^{}]*}//g' | sed -e 's/texttt{[^{}]*}//g' | sed -e 's/url{[^{}]*}//g' | { grep --color=always '\bnovas\b' && echo "DID YOU MEAN novae ?" && exit 1 || true; }
	#
	
check_no_whitespace: $(TEXFILE_BASENAME).tex
	#  cut -f1 -d"%" -- ignore everything after %
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	#
	# period      sed 's:[A-Z].[A-Z].::g' will allow for two capital letter combinations like initials K.S.
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:R.A.::g' | sed 's:L.A.Cosmic::g' | sed 's:\\.M::g' | sed 's:Obs.ID::g' | sed 's:U.S.::g' | sed 's:H.E.S.S.::g' | sed 's:J.D.L.::g' | sed 's:K.V.S.::g' | sed 's:E.A.::g' | sed 's:Ras.Pi::g' | sed 's:Ph.D.::g' | sed 's:P.O.::g' | sed 's:[A-Z].[A-Z].[A-Z].::g'  | sed 's:[A-Z].[A-Z].::g' | { grep --color=always -e '\.[A-Z]' && exit 1 || true; }
	# two periods
	# sed -e 's/\.\.\.//g' -- allow for three periods 
	# sed -e 's/\.\.\///g' -- allow for '../' as in file path
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\.\.\.//g' | sed -e 's/\.\.\///g' | { grep --color=always -e '\.\.' && exit 1 || true; }
	# coma periods;   sed 's:\\,::g' -- remove unbreakable half-spaces from the test
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e '\,\.' && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e ',\.' && exit 1 || true; }
	# some journal styles allow ".," combination: "e.g.,"
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\,' && exit 1 || true; }
	# two comas;   sed 's:\\,::g' -- remove unbreakable half-spaces from the test
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e '\,\,' && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e ',,' && exit 1 || true; }
	#
	# White space between Fig. and ref
	cat *.tex | { grep --color=always 'Fig \\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figs \\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Fig\, \\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figs\. \\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Fig\.\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figs\.\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Fig\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figs\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Fig~\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figs~\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figure\\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figures\\ref' && echo "SHOULD BE Figures~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figure \\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat *.tex | { grep --color=always 'Figures \\ref' && echo "SHOULD BE Figures~\\ref{}" && exit 1 || true; }
	# White space before \cite
	cat *.tex | sed 's:\\protect\\citeauthoryear::g' | sed 's:\\protect\\citename::g' | { grep --color=always '[a-z]\\cite' && echo "NO WHITE SPACE BEFORE \\cite" && exit 1 || true; }

check_extra_white_space: $(TEXFILE_BASENAME).tex
	cat *.tex | cut -f1 -d"%" | grep -v -e '\.\.\/' -e ' \.\/' | { grep --color=always ' \.' && exit 1 || true; }
	cat *.tex | { grep --color=always ' \,' && exit 1 || true; }

check_coma_instead_of_period: $(TEXFILE_BASENAME).tex
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | grep -v -e 'Uni' -e 'Obs' -e 'Inst' -e 'The Netherlands' -e 'The United' | { grep --color=always -e '\,The' -e '\, The' && exit 1 || true; }

check_units: $(TEXFILE_BASENAME).tex
	cat *.tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always '\bhr\b' && echo "SHOULD BE h ACCORDING TO IAU RECOMMENDATIONS ON UNITS https://www.iau.org/publications/proceedings_rules/units/" && exit 1 || true; }

check_phrasing: $(TEXFILE_BASENAME).tex
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\ballow one to identify\b' -e '\ballow to identify\b' && echo "SHOULD BE allow the identification of" && exit 1 || true; }

try_to_find_duplicate_words: $(TEXFILE_BASENAME).tex
	#
	# Checking for repeated words over linebreaks
	# We do not exclude comments, so line numbers will be correct
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	# grep -v ' \-\-[A-Za-z]'    -- remove command line arguments examples
	#                   ' & '    -- ignore tables that may well have duplicate words/numbers
	cat *.tex | grep -v -e ' \--[A-Za-z]' -e ' & ' | cut -f1 -d"%" | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#  sed 's/%.*$//'    -- remove everything after %
	#  sed '/^[[:space:]]*$/d' -- remoove empty lines
	# The output line nubers may not be exact as we skip comment lines
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	cat *.tex | grep -v -e ' \--[A-Za-z]' -e ' & ' | cut -f1 -d"%" | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#
	# Catch word repeats in one line (obsolete)
	# The old version that doesn't catch everything
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	#cat $(TEXFILE_BASENAME).tex | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | grep -v -E '[0-9]cm' | grep -v -E '[0-9]in' | grep -v -e '&' -e 'textwidth' -e 'includegraphicx' -e 'includegraphics' -e 'tabular' | { egrep "(\b[a-zA-Z]+) \1\b"  && exit 1 || true; }
	# The new experimental version
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	# mess 'caption{}' and 'captionbox{}' as we still want to check for repeated words in captions
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	cat *.tex | grep -v -e ' \--' -e ' & ' | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ein --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	# Last-trench effort -- just grep for the most common repetitions
	cat *.tex | { grep --color=always -e ' the the ' -e ' a the ' && exit 1 || true; }
	#
	#######################
	# sed 's/[[:blank:]]\+/ /g' - replace multiple white spaces with one white space
	# Search for suspicious word combinations
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always  "\bare know\b" && exit 1 || true; }
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always -e "\bmission line\b" -e "\bmission lines\b" && exit 1 || true; }
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bwill be also be\b" && exit 1 || true; }
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bdivided my the\b" && exit 1 || true; }
	cat *.tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bthe on\b" && exit 1 || true; }
	# "the were" -> "they were"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bthe were\b' && echo "DID YOU MEAN they were ?" && exit 1 || true; }
	cat *.tex | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bthe were\b' && echo "DID YOU MEAN they were ?" && exit 1 || true; }
	# "Through this paper" -> "Throughout this paper"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bThrough this paper\b' && echo "DID YOU MEAN throughout this paper ?" && exit 1 || true; }
	cat *.tex | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bThrough this paper\b' && echo "DID YOU MEAN throughout this paper ?" && exit 1 || true; }
	# "in order to not" -> "in order not to"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bin order to not\b' && echo "DID YOU MEAN in order not to ?" && exit 1 || true; }	
	cat *.tex | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bin order to not\b' && echo "DID YOU MEAN in order not to ?" && exit 1 || true; }	
	# two version -> two versions
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case -e '\btwo version\b' -e '\bthree version\b' -e '\bfour version\b' -e '\bfive version\b' -e '\bsix version\b' -e '\bseven version\b' -e '\beight version\b' -e '\bnine version\b' -e '\bten version\b' -e '\beleven version\b' -e '\btwleve version\b' && echo "DID YOU MEAN versions ?" && exit 1 || true; }	
	cat *.tex | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case -e '\btwo version\b' -e '\bthree version\b' -e '\bfour version\b' -e '\bfive version\b' -e '\bsix version\b' -e '\bseven version\b' -e '\beight version\b' -e '\bnine version\b' -e '\bten version\b' -e '\beleven version\b' -e '\btwleve version\b' && echo "DID YOU MEAN versions ?" && exit 1 || true; }	
	# minor and minor axes
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case 'minor and minor axes' && echo "DID YOU MEAN major and minor axes ?" && exit 1 || true; }	
	cat *.tex | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case 'minor and minor axes' && echo "DID YOU MEAN major and minor axes ?" && exit 1 || true; }	
	
	
# This hack will modify the .bib file replacing some long journal names if we are using mnras_shortlisthack.bst style
shorten_journal_names_bib: $(BIBFILENAME)
ifeq ($(MODIFY_BIBFILE_ULTRACOMPACT_REF),yes)
	# Modify .bib
	@echo "I WILL RUIN THE BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
	# If the bibfile looks unmodified, save a backup copy
	cat $(BIBFILENAME) | { grep -e '{ATel}' -e '{RNAAS}' -e '{AN}' || cp -v $(BIBFILENAME) $(BIBFILENAME)_backup_long_journal_names ; }
	# Do the actual modification
	cat $(BIBFILENAME) | sed 's:{The Astronomer.s Telegram}:{ATel}:g' | sed 's:{Research Notes of the American Astronomical Society}:{RNAAS}:g' | sed 's:{Astronomische Nachrichten}:{AN}:g' > $(BIBFILENAME)_tmp && mv -v $(BIBFILENAME)_tmp $(BIBFILENAME)
else
	# Nothing to do
	@echo "KEEP THE ORIGINAL BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
endif

check_british_spelling:
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
	# Check for British spelling
	# MNRAS style guide https://academic.oup.com/mnras/pages/General_Instructions#6%20Style%20guide
	cat *.tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'timescale' && echo "SHOULD BE time-scale" && exit 1 || true; }
	# random collection of astronomy-specific words
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'barycenter' && echo "SHOULD BE barycentre" && exit 1 || true; }
	# random collection of words
	# sed 's/\\[^~]*{//g'  will remove \textcolor{
	cat *.tex | cut -f1 -d"%" | sed 's/\\[^~]*{//g' | grep -v -e 'xcolor' -e 'rgbcolor' | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat *.tex | cut -f1 -d"%" | sed 's:laborator::g' | sed 's:ollaboration::g' | grep -v '$^{' | { grep --color=always '\blabor\b' && echo "SHOULD BE labour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case '\banalog\b' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'centimeter' && echo "SHOULD BE centimetre" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	# Other MNRAS things
	# https://academic.oup.com/mnras/pages/general_instructions#6.5%20Miscellaneous%20journal%20style
	cat *.tex | { grep --color=always --ignore-case -e '\\%' -e 'percent' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\,' && echo "SHOULD BE e.g." && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\.\,' && echo "SHOULD BE i.e." && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case '``' && echo "SHOULD BE \`" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case "''" && echo "SHOULD BE \'" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'eq\.' -e 'eqn\.' -e 'Eq\.' -e 'Eqn\.' && echo "SHOULD BE equation~()" && exit 1 || true; }
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE A MNRAS MANUSCRIPT - NOT ENFORCING BRITISH SPELLING"
	echo $(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING)
endif

check_us_spelling:
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
	# Check for US spelling
	# AAS style guide https://journals.aas.org/aas-style-guide/
	# they also suggest follow The Chicago Manual of Style https://www.chicagomanualofstyle.org/home.html
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centred' && echo "SHOULD BE centered" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centre' && echo "SHOULD BE center" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulphur' && echo "SHOULD BE sulfur" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labelled' && echo "SHOULD BE labeled" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyse' && echo "SHOULD BE analyze" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrized' && echo "SHOULD BE parameterized" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrize' && echo "SHOULD BE parametrise" && exit 1 || true; }
	# Why I was under impression that 'acknowledgements' is the correct spelling in AAS journals?
	# Their style guide spells 'acknowledgments' https://journals.aas.org/manuscript-preparation/#acknowledgments
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgements' && echo "SHOULD BE acknowledgments" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artefact' && echo "SHOULD BE artifact" && exit 1 || true; }
	# Yes, best-fitting seems to be OK at AAS
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fitting ' && echo "SHOULD BE best-fit" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e ' disc\,' -e ' disc\.' -e 'disc$$' -e 'disc ' && echo "SHOULD BE disk" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'haloes' && echo "SHOULD BE halos" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' on to ' && echo "SHOULD BE onto" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'time-scale' && echo "SHOULD BE timescale" && exit 1 || true; }
	#
	# random collection of words
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'colour' && echo "SHOULD BE color" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavour' && echo "SHOULD BE flavor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humour' && echo "SHOULD BE humor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labour' && echo "SHOULD BE labor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbour' && echo "SHOULD BE neighbor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyse' && echo "SHOULD BE paralyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalogue' && echo "SHOULD BE catalog" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analogue' && echo "SHOULD BE analog" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modelling' && echo "SHOULD BE modeling" && exit 1 || true; }
	# Other AAS things
	#cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\. ' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\]' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\. ' && echo "SHOULD BE i.e.," && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' `[a-zA-Z]' && echo "SHOULD BE \`\`" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | grep -v "s' " | { grep --color=always --ignore-case "[a-zA-Z]' " && echo "SHOULD BE \'\'" && exit 1 || true; }
	# super AAS-specific
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'Fig\.' && echo "SHOULD BE Figure" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'Figs\.' && echo "SHOULD BE Figures" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'Sec\.' && echo "SHOULD BE Section" && exit 1 || true; }
	#
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'errorbar' && echo "SHOULD BE error bar" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'free-fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'free fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'free~fall' && echo "SHOULD BE freefall" && exit 1 || true; }
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE AN AAS MANUSCRIPT - NOT ENFORCING US SPELLING"
	echo $(AAS_MANUSCRIPT_REQUIRING_US_SPELLING)
endif

# We want to check for a consistent use of 'gamma-ray' vs '$\gamma$-ray', but only if it's a journal paper:
# in a proposal draft we may have an ASCII-only abstract and LaTeX text body.
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=no
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=yes
endif
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=yes
endif
check_gamma_ray_math_mode:
ifeq ($(DO_IT_CHECK_GAMMA_RAY_MATH_MODE),yes)
	@echo "THIS IS AN MNRAS OR AAS MANUSCRIPT"
	echo $(DO_IT_CHECK_GAMMA_RAY_MATH_MODE)
	{ cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --quiet 'gamma-ray' && cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --quiet '$$\\gamma$$-ray' && cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --color=always -e 'gamma-ray' -e '$$\\gamma$$-ray' && echo "SHOULD BE USING CONSISTENTLY 'gamma-ray' or '$$\\gamma\$$-ray'" && exit 1 || true; }
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE AN MNRAS OR AAS MANUSCRIPT - NOT ENFORCING MATH MODE for 'gamma-ray'"
	echo $(DO_IT_CHECK_GAMMA_RAY_MATH_MODE)
endif

check_software_small_capitals:
ifeq ($(ANY_KNOWN_SOFTWARE_MENTIONED),yes)
ifeq ($(TEST_SOFTWARE_TEXTSC),yes)
	# Check that \textsc is used in the text
	@echo "CHECK IF \\textsc{SoftWare} IS USED"
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -e '\\textsc' -e '\\scshape'
endif
else
	# Nothing to do
	@echo "NO KNOWN SOFTWARE NAMES RECOGNIZED"
	echo $(ANY_KNOWN_SOFTWARE_MENTIONED)
endif

check_swift_uvot_lowercase_filternames:
ifeq ($(IS_SWIFT_UVOT_MENTIONED),yes)
	# Check that Swift/UVOT filter names are lowercase
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'UVW1' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvw1 ?" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'UVM2' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvm2 ?" && exit 1 || true; }
	cat *.tex | cut -f1 -d"%" | { grep --color=always 'UVW2' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvw2 ?" && exit 1 || true; }
else
	# Nothing to do
	@echo "NO MENTION OF SWIFT UVOT"
	echo $(IS_SWIFT_UVOT_MENTIONED)
endif

check_consistent_unbreakable_space_size_UT:
	{ cat *.tex | cut -f1 -d"%" | grep --quiet '~UT' && cat *.tex | cut -f1 -d"%" | grep --quiet '\\\,UT' && cat *.tex | cut -f1 -d"%" | grep --color=always -e '~UT' -e '\\\,UT' && echo "SHOULD BE USING CONSISTENTLY '~UT' or '\\,UT" && exit 1 || true; }

check_filenames_good_for_arXiv:
	# Check if all filenames in the current directory contain only characters that are good for arXiv
	# as listed at https://info.arxiv.org/help/submit/index.html#files
	{ for FILENAME in * ;do if [[ "$$FILENAME" =~ ^[0-9A-Za-z_\\.\\,\-\\=\\+]+$$ ]]; then echo "The filename '$$FILENAME' looks good"; else echo "The filename '$$FILENAME' has characters not good for arXiv"; fi ;done | grep --color=always 'characters not good for arXiv' && exit 1 || true; }



$(TEXFILE_BASENAME).pdf: $(TEXFILE_BASENAME).tex
ifeq ($(PDFTEX),yes)
	# pdflatex
	@echo "YES PDF"
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	@echo "YES BibTeX"
	echo $(BIBTEX)
	# This works with .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex 
endif
else
	@echo "NO BibTeX"
	echo $(BIBTEX)
	# No BibTeX, .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex 
endif
endif

else
	# latex
	@echo "NO PDF  "
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	@echo "YES BibTeX"
	echo $(BIBTEX)
	# BibTeX and .eps figures (the right way)
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && latex $(TEXFILE_BASENAME).tex && { latex $(TEXFILE_BASENAME).tex 2>&1 | grep --color=always 'undefined on input line' && exit 1 || true; } && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex 
endif
else
	@echo "NO BibTeX"
	echo $(BIBTEX)	
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex 
endif
endif

endif


check_for_bonus_figures: $(TEXFILE_BASENAME).tex
	{ for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat *.tex | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; }  && { cat *.tex | cut -f1 -d'%' | grep 'label{fig:' | awk -F'label{' '{print $$2}' | awk -F'}' '{print $$1}' | while read LABELLED_FIGURE ; do cat *.tex | cut -f1 -d'%' | grep --quiet "ref{$$LABELLED_FIGURE}" && continue ; echo "WARNING: a figure not referenced in the main text: $$LABELLED_FIGURE" ;done ; echo " " ; }


display_compiled_pdf: $(TEXFILE_BASENAME).pdf
	@echo "The document is successfully compiled: "$(TEXFILE_BASENAME).pdf
ifeq ($(LAUNCH_OKULAR_PDF_VIEWER_TO_DISPLAY_COMPILED_PAPER),yes)
	@echo "Starting Okular PDF viewer to display "$(TEXFILE_BASENAME).pdf
	okular $(TEXFILE_BASENAME).pdf
endif

